A Deontic Logic Analysis of Autonomous Systems' Safety

We consider the pressing question of how to model, verify, and ensure that autonomous systems meet certain \textit{obligations} (like the obligation to respect traffic laws), and refrain from impermissible behavior (like recklessly changing lanes). Temporal logics are heavily used in autonomous system design; however, as we illustrate here, temporal (alethic) logics alone are inappropriate for reasoning about obligations of autonomous systems. This paper proposes the use of Dominance Act Utilitarianism (DAU), a deontic logic of agency, to encode and reason about obligations of autonomous systems. We use DAU to analyze Intel's Responsibility-Sensitive Safety (RSS) proposal as a real-world case study. We demonstrate that DAU can express well-posed RSS rules, formally derive undesirable consequences of these rules, illustrate how DAU could help design systems that have specific obligations, and how to model-check DAU obligations.

==> chapters/apxDefnObligation.tex <==

\section{The definition of obligation statements}
\label{apx:proof of many dstits}
In Def.~\ref{def:obligation structure}, there is no loss in generality in only allowing one positive $dstit$ in an obligation (i.e., not preceded by a negation), as shown by the following result:
\begin{proposition}
	\label{prop:many dstits}
	Where $\formula\in$ \CTLs, it holds that
	$\dstit{\alpha}{\dstit{\alpha}{\formula}} \equiv \dstit{\alpha}{\formula}$
\end{proposition}

\begin{proof}
	Let $\xi = \dstit{\alpha}{\dstit{\alpha}{\formula}}$.
	For a history $h\in H_m$, recall that $\Choiceam(h)$ is the unique action $K$ at $m$ s.t. $h\in K$,
	and that $K$ is itself a set of histories.
	%Let $\Nhbram(h) \subset H_m$ be the set of histories in $K$.
	E.g. in Fig.~\ref{fig:tree opposite}, $\Choiceam(h_1)=K_1 = \{h_1,h_2,h_3\}$.
	Note that $\Choiceam(h)$ is never empty since $h\in \Choiceam(h)$.
	
	%First we prove $\xi \equiv \dstit{\alpha}{\formula}$.
	Let $m/h$ be a pair in a model $\Model$.
	By definition, 
	\begin{equation}
	\label{eq:xi}
	m/h\models \xi \text{ iff } \Choiceam(h) \subseteq |\dstit{\alpha}{\formula}|_m \text{ and } H_m\neq |\dstit{\alpha}{\formula}|_m
	\end{equation}
	We have
	\[|\dstit{\alpha}{\formula}|_m = \left \lbrace\begin{matrix}\{h'\such \Choiceam(h') \subseteq  |\formula|_m\} \defeq \Choiceam(\formula), &\quad& H_m \neq |\formula|_m \\ \emptyset, & \quad& H_m = |\formula|_m \end{matrix}\right.\]
	%
	$\Choiceam(\formula)$ is the set of histories whose actions at $m$ guarantee $\formula$.
	In Fig.~\ref{fig:tree opposite} $\Choiceam(\psi)=\Choiceam(\chi)=\{h_1,h_2,h_3\}$ while $\Choiceam(\varphi_1)=\emptyset$.
	In general, $\Choiceam(\formula)\subseteq |\formula|_m$.
	
	Now if $H_m=|\formula|_m$, \eqref{eq:xi} implies $\Choiceam(h) \subseteq \emptyset$ which is impossible.
	Therefore $m/h\models \xi$ iff $H_m\neq |\formula|_m$, $\Choiceam(h) \subseteq \Choiceam(\formula)$ and $H_m \neq \Choiceam(\formula)$.
	We now show these three conditions are equivalent to $m/h\models \dstit{\alpha}{\formula}$.
	
	$(\implies)$ Since $\Choiceam(\formula) \subseteq |\formula|_m$ then $\Choiceam(h) \subseteq |\formula|_m$, and combined with $H_m\neq |\formula|_m$this is the definition of $m/h\models \dstit{\alpha}{\formula}$.
	
	$(\Rightarrow)$ For the converse, suppose $H_m\neq |\formula|_m$ and $\Choiceam(h) \subseteq |\formula|_m$.
	Then a fortiori $H_m\neq \Choiceam(\formula)$ and $\Choiceam(h) \subseteq \Choiceam(\formula)$ because actions partition $H_m$. 
	\hspace*{\fill}QED.
\end{proof}

%%%%%%%%%%%%%%	
%The proof for $\dstit{\alpha}{\neg \dstit{\alpha}{\formula}} \equiv \dstit{\alpha}{\neg \formula}$ proceeds along similar lines.
%%
%Set $\zeta = \dstit{\alpha}{\neg \dstit{\alpha}{\formula}}$.
%Let $m/h$ be a pair in a model $\Model$.
%By definition, 
%\begin{equation}
%\label{eq:zeta}
%m/h\models \zeta \text{ iff } \Choiceam(h) \subseteq |\neg \dstit{\alpha}{\formula}|_m \text{ and } H_m\neq |\neg \dstit{\alpha}{\formula}|_m
%\end{equation}
%%
%We have
%\[ |\neg \dstit{\alpha}{\formula}|_m = \overline{|\dstit{\alpha}{\formula}|_m}=\left \lbrace
%\begin{matrix} 
%\overline{\Choiceam(\formula)}, &\quad& H_m \neq |\formula|_m \\ 
%\overline{\emptyset} = H_m, & \quad& H_m = |\formula|_m 
%\end{matrix}\right.\]
%
%Now if$H_m=|\formula|_m$ then \eqref{eq:zeta} implies $H_m\neq H_m$.
%Therefore $m/h\models \zeta$ iff $H_m \neq |\formula|_m$, $\Choiceam(h) \subseteq \overline{\Choiceam(\formula)}$ and $H_m \neq \overline{\Choiceam(\formula)}$.
%%
%We now show these three conditions are equivalent to $m/h\models \dstit{\alpha}{\neg \formula}$.
%
%$(\Rightarrow)$ Since $\Choiceam(\formula) \subseteq |\formula|_m$ then $\Choiceam(h)\cap |\formula|_m=\emptyset$ so $\Choiceam(h)$ guarantees  $\neg \formula$. 
%From $H_m \neq \overline{\Choiceam(\formula)}$ we conclude that $H_m$ contains some histories whose actions guarantee $\formula$ and a fortiori some histories satisfy $\formula$, so $H_m \neq |\neg \formula|_m$.
%These two conclusions define $m/h\models \dstit{\alpha}{\neg \formula}$.
%
%$(\Leftarrow)$ For the converse, suppose $H_m\neq |\neg \formula|_m$ and $\Nhbram(h) \subseteq \overline{|\formula|_m}$.
%Then $\Choiceam(h) \subseteq \overline{\Choiceam(\formula)}$.
%Moreover, since every history in $\Choiceam(h)$ violates $\formula$ at $m$, then the action $\Choiceam(h)$ guarantees $\neg \formula$, 
%QED.

==> chapters/apxProofModelInference.tex <==
\section{Proof of Prop.~\ref{prop:stit model inference}}
\label{apx:proof of stit model inference}

In this proof we let $[m:n]$ denote the set of integers $\{m,m+1,\ldots, n\}$, and we simplify the notation by writing $g$ and $p$ instead of $g_\alpha$ and $p_\alpha$ for the atomic propositions `$\alpha$ is granted right-of-way' and `$\alpha$ passes through the conflict region', respectively.
%
Starting with $\rssass$, let $A= \neg p \wbuntil g$.
The set of histories $|\dstit{\alpha}{A}|_m = \{h\such m/h\models \dstit{\alpha}{A}\} = \{h \such \Choiceam(h)\subseteq |A|_m\}$ if $H_m\neq|A|_m$, and is empty otherwise. 
Since the case when it is empty is trivial, we focus on the first case in what follows.
Therefore $|\neg\dstit{\alpha}{A}|_m = \{h \such \Choiceam(h) \nsubseteq |A|_m\}$.
%
Now Eq.~\eqref{eq:rss-assertive} says that $\forall K\in \Optimalam/w_\alpha$, $K\subseteq \{h\such \Choiceam(h)\nsubseteq |A|_m\}$, which is equivalent to $K \nsubseteq |A|_m$ (since $\Choiceam(h) = K$ for every $h\in K$).
So for all $K\in \Optimalam/w_\alpha$, $\exists h \in K$ s.t. $m/h \not\models \neg p \wbuntil g$.
From the semantics of $\wbuntil$, this is equivalent to : for all $K\in \Optimalam/w_\alpha$,
\[\exists \tilde{h} \in K \text{ s.t. } \exists i\in [m:m+N]~.~i'/\tilde{h}\models \neg g \forall i' \in [m:i] \text{ but } i''/\tilde{h} \models p \text{ for some } i''\in [m:i] \]

So $i''/\tilde{h}\models p \land \neg g$ and $m/\tilde{h}\models \neg g$, so $m/\tilde{h}\not\models \always(\neg g \implies \neg p)$.
%Moreover $m/\tilde{h}\models \neg g \implies K\cap |\neg g|_m \neq \emptyset \implies K \in \Optimalam/\neg g$.
%Thus a choice of $K$ at $m$ is consistent with both obligations.
If the system evolves along $\tilde{h}$, it risks violating $\rssrow$ at $i''$.
To avoid this, $\tilde{h}$ must not be in any of the optimal actions of $\Optimal{\alpha}{m'}$.
So the $\Value$ function must be designed so that $\Choice{\alpha}{m'}(\tilde{h}) \prec K_3$ for some $K_3 \in \Optimal{\alpha}{m'}$, as shown in Fig.~\ref{fig:derive policies}.
From this we conclude $|\Choice{\alpha}{m'}|\geq 2$ and $|K_1|\geq 2$.
\hspace*{\fill}QED.

==> chapters/apxProofThm1.tex <==
\section{Proof  of Thm.~\ref{thm:force others}}
\label{apx:proof force others}
	Assume that $m/h \models \Ostit{\alpha}{A \lor B} \land \forall \neg A$.
	By definition of the dominance ought, 
	for all $K \in \Optimalam, K\subseteq |A\lor B|_m$.
	And by definition of $|A|_m$ (Eq.~\ref{eq:Amm}), $|A\lor B|_m = |A|_m \cup |B|_m$.
	We also have that $m/h\models \forall \neg A$, i.e., $m/h' \models \neg A$ for all $h' \in H_m$; thus $|A|_m = \emptyset$.
	Therefore $\forall K \in \Optimalam, K\subseteq |B|_m$, which is the definition of $m/h \models \Ostit{\alpha}{B}$.
\hspace*{\fill}QED.

==> chapters/apxRSS1notmet.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof that $RSS$\ref{rss-behind} cannot be satisfied in some cases}
\label{apx:rss-behind}
We show that if a rear-end collision is unavoidable, then formula $RSS$\ref{rss-behind} can't be satisfied.
Indeed, since $H_m=|B|_m$, then $\Optimalam \subset |B|_m$.
By definition of $\neg B$, $|\neg B|_m = H_m \setminus |B|_m = \emptyset$. 
Thus $\Optimalam=\emptyset$ and no optimal action can satisfy $\neg B$, so the obligation cannot be met.

==> chapters/computevn.tex <==

\subsection{Computing the extremal values $\vnl$ and $\vnu$}
\label{sec:computing vn}
%We use the letter $e$ to denote a generic transition. 
%In the construction of the previous section, an execution $\pi$ of $T$ maps to a history $h$ in $\Model_T$ and $w(\pi)$ is taken as the definition of $\Value(h)$.
%Then $\vnu = \sup \{w(\pi) \such \pi \in E(\strategy)\}$.

The question we answer in this section is: how to compute $\vnu$?
(Computation of $\vnl$ is similar).
Clearly, the answer depends on the function $\lambda$ used for accumulating weights along an execution: e.g., if $\lambda$ is addition and all the weights are positive, then all executions have infinite value, and every future is ideal, which is a comforting thought but of little interest in modeling the real world.
There are several instantiations of $\lambda$ that can model real-world phenomena, and lead to finite values of $\vnu$.
Here we give one example, and leave others to a longer version of the paper.

An infinite execution visits at least one cycle in $T$ infinitely many times. 
There is a finite number of cycles in $T$ but infinitely many ways to traverse them in a given execution; e.g., for 2 cycles $C_1$ and $C_2$ sharing a state, two schedules for traversing them are
$\Sigma_1: \pi C_1C_2C_1C_2\ldots$ and $\Sigma_2: \pi C_1C_2C_1C_1C_2C_1C_1C_1C_2\ldots$; $\pi$ is a finite prefix leading to $C_1$.
We would like $\lambda$ to be such that 
\begin{equation}
\label{eq:lambda}
\lambda(\Sigma_1) = \lambda(\Sigma_2) = \lambda(\pi)\otimes \lambda(C_1^+)\otimes \lambda(C_2^+)
\end{equation}
According to Eq.~\eqref{eq:lambda}, the utility depends only on which cycles are in the schedule, and can be computed by combining (via some commutative operation $\otimes$) the utility of traversing $C_1$ infinitely many times with that of traversing $C_2$ infinitely many times, with the utility of traversing the prefix $\pi$.
We refer to $(\pi,C_1,C_2)$ as an \textit{abstract schedule.}
%
If $\lambda$ is such, then even though there is an infinite number of executions, they fall into a finite number of abstract schedules, and all executions in a given abstract schedule have equal value. 
Presumably, $\lambda(C^+)$ is computable.

%
%Take $\lambda$ to be $\liminfavg$, defined as
%$\liminfavg(a_0a_1a_2\ldots) \defeq \liminf_n (a_n/n)$.
%It is the infimum of the  accumulation points of sequence $a_n$.
%E.g. if $w(e)$ is the time-to-collision following the action in transition $e$, then $\Value(h)$ is, roughly, the long-term average time-to-collision.%\footnote{We use $\liminf$, instead of $\lim$, because it always exists}
%Or, if $w(e)$ is the robustness of the dynamical trajectory that follows from an action relative to some temporal logic specification~\cite{FainekosP09tcs}, then $\Value(h)$ is the long-term average robustness.

Take $\lambda = \min$ as an example. 
Clearly, this satisfies Eq.~\eqref{eq:lambda} with $\otimes = \min$. 
For instance, if $w((q,K,q'))$ is the time-to-collision resulting from action $K$ then $\Value(h)$ is the shortest time-to-collision encountered along the history, and an optimal history is one with the highest minimum time-to-collision.
It's a simple matter to prove that $\vnu$ is the maximum weight of any reachable transition from $q_0$, which can be computed in a finite number of steps.
(Unfortunately, different $\lambda$s will, in general, require different customized proofs that they satisfy Eq.~\eqref{eq:lambda}.)

How do we find the abstract schedules?
An abstract schedule consists of a finite prefix in $T$, followed by a \textit{finite} sequence of cycles (possibly with finite paths connecting them if they don't share a state.)
Therefore, create a new automaton $U$ with unlabeled edges as follows:
1) Set $U.q_0 = T.q_0$.
2) To every cycle $C$ in $T$, add a new state $q_C$ to $U$.
3) If there's a path connecting $C$ and $C'$, add that path between $q_C$ and $q_{C'}$ with the same weights.
4) If $C$ and $C'$ share a state, add a transition $(q_C,q_{C'})$ to $U$ with weight 0.
5) To every path between $T.q_0$ and a cycle $C$, add a similar path between $U.q_0$ and $q_C$, with the same weights.

Now every finite path in $U$ \textit{with at most one cycle in it} represents an abstract schedule in $T$, and these can be found in finite time.

==> mypackages.tex <==
% PACKAGES
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{ifthen}
\usepackage{color,soul}
\usepackage{txfonts}
\usepackage[linesnumbered]{algorithm2e}
% \usepackage{MnSymbol}

% \usepackage{times}
\usepackage{fullpage}
\usepackage{url}
\usepackage{tikz}
\usetikzlibrary{arrows,backgrounds,decorations,decorations.pathmorphing,
	positioning,fit,automata,shapes,snakes,patterns,plotmarks,calc,trees}
%\usepackage[dvips]{graphicx}
\usepackage{subfig}
\usepackage{latexsym}	
\usepackage{xspace}
\usepackage{alltt}
\usepackage[obeyFinal]{todonotes}
\usepackage{wrapfig}
%\usepackage{subcaption}
\usepackage[per-mode=symbol]{siunitx}
\usepackage{paralist}
\usepackage[shortlabels]{enumitem}
\usepackage{color,colortbl}
\usepackage{pgfgantt}

% \usepackage{amsfonts}
\usepackage{epsfig,color}
\usepackage{algpseudocode}
% \usepackage[ruled]{algorithm}
\usepackage{mdwlist}% Compact list formats \itemize*, \enumerate*
\usepackage{setspace} % This must precede hyperref
\usepackage{hyperref}
\usepackage[depth=1]{bookmark}
\usepackage{listings}
\usepackage{caption}
\usepackage{xspace}
\usepackage{tikz}
\usepackage{stmaryrd}
\usepackage{multirow}
\usepackage{ltl}
